Skyrmionic Spin Structures in Layered Fe5GeTe2 Up To Room Temperature

The role of the crystal lattice, temperature and magnetic field for the spin structure formation in the 2D van der Waals magnet Fe5GeTe2 is a key open question. Using Lorentz transmission electron microscopy, we experimentally observe topological spin structures up to room temperature in the metastable pre-cooling and stable post-cooling phase of Fe5GeTe2. Over wide temperature and field ranges, skyrmionic magnetic bubbles form without preferred chirality, which is indicative of a centrosymmetric crystal structure. In the pre-cooling phase, these bubbles are observable even without the application of an external field, while in the post-cooling phase, a transformation from bubble domains to stripe domains is seen. To understand the magnetic order in Fe5GeTe2 we compare macroscopic magnetometry characterization results with microscopic density functional theory calculation. Our results show that even up to room temperature, topological spin structures can be stabilized in centrosymmetric van der Waals magnets.

==> literature.tex <==
% This file was created with Citavi 6.8.0.0

@article{Gibertini.2019,
 abstract = {The family of two-dimensional (2D) materials grows day by day, hugely expanding the scope of possible phenomena to be explored in two dimensions, as well as the possible van der Waals (vdW) heterostructures that one can create. Such 2D materials currently cover a vast range of properties. Until recently, this family has been missing one crucial member: 2D magnets. The situation has changed over the past 2 years with the introduction of a variety of atomically thin magnetic crystals. Here we will discuss the difference between magnetic states in 2D materials and in bulk crystals and present an overview of the 2D magnets that have been explored recently. We will focus on the case of the two most studied systems-semiconducting CrI3 and metallic Fe3GeTe2-and illustrate the physical phenomena that have been observed. Special attention will be given to the range of new van der Waals heterostructures that became possible with the appearance of 2D magnets, offering new perspectives in this rapidly expanding field.},
 author = {Gibertini, M. and Koperski, M. and Morpurgo, A. F. and Novoselov, K. S.},
 year = {2019},
 title = {Magnetic 2D materials and heterostructures},
 pages = {408--419},
 volume = {14},
 number = {5},
 journal = {Nature nanotechnology},
 doi = {10.1038/s41565-019-0438-6},
 file = {http://www.ncbi.nlm.nih.gov/pubmed/31065072}
}


% This file was created with Citavi 6.8.0.0

@article{Huang.2017,
 abstract = {Since the discovery of graphene, the family of two-dimensional materials has grown, displaying a broad range of electronic properties. Recent additions include semiconductors with spin-valley coupling, Ising superconductors that can be tuned into a quantum metal, possible Mott insulators with tunable charge-density waves, and topological semimetals with edge transport. However, no two-dimensional crystal with intrinsic magnetism has yet been discovered; such a crystal would be useful in many technologies from sensing to data storage. Theoretically, magnetic order is prohibited in the two-dimensional isotropic Heisenberg model at finite temperatures by the Mermin-Wagner theorem. Magnetic anisotropy removes this restriction, however, and enables, for instance, the occurrence of two-dimensional Ising ferromagnetism. Here we use magneto-optical Kerr effect microscopy to demonstrate that monolayer chromium triiodide (CrI3) is an Ising ferromagnet with out-of-plane spin orientation. Its Curie temperature of 45 kelvin is only slightly lower than that of the bulk crystal, 61 kelvin, which is consistent with a weak interlayer coupling. Moreover, our studies suggest a layer-dependent magnetic phase, highlighting thickness-dependent physical properties typical of van der Waals crystals. Remarkably, bilayer CrI3 displays suppressed magnetization with a metamagnetic effect, whereas in trilayer CrI3 the interlayer ferromagnetism observed in the bulk crystal is restored. This work creates opportunities for studying magnetism by harnessing the unusual features of atomically thin materials, such as electrical control for realizing magnetoelectronics, and van der Waals engineering to produce interface phenomena.},
 author = {Huang, Bevin and Clark, Genevieve and Navarro-Moratalla, Efr{\'e}n and Klein, Dahlia R. and Cheng, Ran and Seyler, Kyle L. and Zhong, Ding and Schmidgall, Emma and McGuire, Michael A. and Cobden, David H. and Yao, Wang and {Di Xiao} and Jarillo-Herrero, Pablo and Xu, Xiaodong},
 year = {2017},
 title = {Layer-dependent ferromagnetism in a van der Waals crystal down to the monolayer limit},
 pages = {270--273},
 volume = {546},
 number = {7657},
 journal = {Nature},
 doi = {10.1038/nature22391},
 file = {http://www.ncbi.nlm.nih.gov/pubmed/28593970}
}


% This file was created with Citavi 6.8.0.0

@article{Deng.2018,
 abstract = {Materials research has driven the development of modern nano-electronic devices. In particular, research in magnetic thin films has revolutionized the development of spintronic devices1,2 because identifying new magnetic materials is key to better device performance and design. Van der Waals crystals retain their chemical stability and structural integrity down to the monolayer and, being atomically thin, are readily tuned by various kinds of gate modulation3,4. Recent experiments have demonstrated that it is possible to obtain two-dimensional ferromagnetic order in insulating Cr2Ge2Te6 (ref. 5) and CrI3 (ref. 6) at low temperatures. Here we develop a device fabrication technique and isolate monolayers from the layered metallic magnet Fe3GeTe2 to study magnetotransport. We find that the itinerant ferromagnetism persists in Fe3GeTe2 down to the monolayer with an out-of-plane magnetocrystalline anisotropy. The ferromagnetic transition temperature, Tc, is suppressed relative to the bulk Tc of 205 kelvin in pristine Fe3GeTe2 thin flakes. An ionic gate, however, raises Tc to room temperature, much higher than the bulk Tc. The gate-tunable room-temperature ferromagnetism in two-dimensional Fe3GeTe2 opens up opportunities for potential voltage-controlled magnetoelectronics7-11 based on atomically thin van der Waals crystals.},
 author = {Deng, Yujun and Yu, Yijun and Song, Yichen and Zhang, Jingzhao and Wang, Nai Zhou and Sun, Zeyuan and Yi, Yangfan and Wu, Yi Zheng and Wu, Shiwei and Zhu, Junyi and Wang, Jing and Chen, Xian Hui and Zhang, Yuanbo},
 year = {2018},
 title = {Gate-tunable room-temperature ferromagnetism in two-dimensional Fe3GeTe2},
 pages = {94--99},
 volume = {563},
 number = {7729},
 journal = {Nature},
 doi = {10.1038/s41586-018-0626-9},
 file = {93904530-bc08-45bd-b358-56ef9530b3e5:C\:\\Users\\Morris\\AppData\\Local\\Swiss Academic Software\\Citavi 6\\ProjectCache\\k4a9175chg9k578gwv8a52s6g23e9do0zsq8mv1wf6n9yo3cr\\Citavi Attachments\\93904530-bc08-45bd-b358-56ef9530b3e5.pdf:pdf}
}


% This file was created with Citavi 6.8.0.0

@article{May.2019,
 abstract = {Two-dimensional materials with intrinsic functionality are becoming increasingly important in exploring fundamental condensed matter science and for developing advanced technologies. Bulk crystals that can be exfoliated are particularly relevant to these pursuits as they provide the opportunity to study the role of physical dimensionality and explore device physics in highly crystalline samples and designer heterostructures in a routine manner. Magnetism is a key element in these endeavors; however, relatively few cleavable materials are magnetic and none possess magnetic order at ambient conditions. Here, we introduce Fe5- xGeTe2 as a cleavable material with ferromagnetic behavior at room temperature. We established intrinsic magnetic order at room temperature in bulk crystals ([Formula: see text] = 310 K) through magnetization measurements and in exfoliated, thin flakes ([Formula: see text] $\approx$ 280 K) using the anomalous Hall effect. Our work reveals Fe5GeTe2 as a prime candidate for incorporating intrinsic magnetism into functional van der Waals heterostructures and devices near room temperature.},
 author = {May, Andrew F. and Ovchinnikov, Dmitry and Zheng, Qiang and Hermann, Raphael and Calder, Stuart and Huang, Bevin and Fei, Zaiyao and Liu, Yaohua and Xu, Xiaodong and McGuire, Michael A.},
 year = {2019},
 title = {Ferromagnetism Near Room Temperature in the Cleavable van der Waals Crystal Fe5GeTe2},
 pages = {4436--4442},
 volume = {13},
 number = {4},
 journal = {ACS nano},
 doi = {10.1021/acsnano.8b09660},
 file = {http://www.ncbi.nlm.nih.gov/pubmed/30865426}
}


% This file was created with Citavi 6.8.0.0

@article{Li.2020,
 abstract = {The van der Waals ferromagnet Fe5GeTe2 has a Curie temperature TC of about 270~K, which is tunable through controlling the Fe deficiency content and can even reach above room temperature. To achieve insights into its ferromagnetic exchange that gives the high TC, the critical behavior has been investigated by measuring the magnetization in Fe5GeTe2 crystal around the ferromagnetic ordering temperature. The analysis of the measured magnetization by using various techniques harmonically reached to a set of reliable critical exponents with TC = 273.7~K, \textgreek{b}~=~0.3457 $\pm$ 0.001, \textgreek{g}~=~1.40617 $\pm$ 0.003, and \textgreek{d}~=~5.021 $\pm$ 0.001. By comparing these critical exponents with those predicted by various models, it seems that the magnetic properties of Fe5GeTe2 could be interpreted by a three-dimensional magnetic exchange with the exchange distance decaying as J(r)~$\approx$~r-4.916, close to that of a three-dimensional Heisenberg model with long-range magnetic coupling.},
 author = {Li, Zhengxian and Xia, Wei and Su, Hao and Yu, Zhenhai and Fu, Yunpeng and Chen, Leiming and Wang, Xia and Yu, Na and Zou, Zhiqiang and Guo, Yanfeng},
 year = {2020},
 title = {Magnetic critical behavior of the van der Waals Fe5GeTe2 crystal with near room temperature ferromagnetism},
 pages = {15345},
 volume = {10},
 number = {1},
 journal = {Scientific Reports},
 doi = {10.1038/s41598-020-72203-3},
 file = {21d442d1-3fa3-4e78-8068-f917e28aa1ef:C\:\\Users\\Morris\\AppData\\Local\\Swiss Academic Software\\Citavi 6\\ProjectCache\\k4a9175chg9k578gwv8a52s6g23e9do0zsq8mv1wf6n9yo3cr\\Citavi Attachments\\21d442d1-3fa3-4e78-8068-f917e28aa1ef.pdf:pdf}
}


% This file was created with Citavi 6.8.0.0

@incollection{Manchon.2017,
 author = {Manchon, Aur{\'e}lien and Belabbes, Abderrezak},
 title = {Spin-Orbitronics at Transition Metal Interfaces},
 pages = {1--89},
 volume = {68},
 publisher = {{Elsevier Science}},
 isbn = {9780128119914},
 series = {Solid State Physics},
 editor = {Stamps, Robert L. and Camley, Robert E.},
 booktitle = {Solid State Physics},
 year = {2017},
 address = {Saint Louis},
 doi = {10.1016/bs.ssp.2017.07.001},
 file = {0cdd0a5c-1a7b-4612-8200-72397c13657c:C\:\\Users\\Morris\\AppData\\Local\\Swiss Academic Software\\Citavi 6\\ProjectCache\\k4a9175chg9k578gwv8a52s6g23e9do0zsq8mv1wf6n9yo3cr\\Citavi Attachments\\0cdd0a5c-1a7b-4612-8200-72397c13657c.pdf:pdf}
}


% This file was created with Citavi 6.8.0.0

@article{Stahl.2018,
 author = {Stahl, Juliane and Shlaen, Evgeniya and Johrendt, Dirk},
 year = {2018},
 title = {The van der Waals Ferromagnets Fe 5-\textgreek{d} GeTe 2 and Fe 5-\textgreek{d}-x Ni x GeTe 2 - Crystal Structure, Stacking Faults, and Magnetic Properties},
 pages = {1923--1929},
 volume = {644},
 number = {24},
 issn = {00442313},
 journal = {Zeitschrift f{\"u}r anorganische und allgemeine Chemie},
 doi = {10.1002/zaac.201800456}
}


% This file was created with Citavi 6.8.0.0

@article{Lemesh.2018,
 abstract = {Magnetic skyrmions promise breakthroughs in future memory and computing devices due to their inherent stability and small size. Their creation and current driven motion have been recently observed at room temperature, but the key mechanisms of their formation are not yet well-understood. Here it is shown that in heavy metal/ferromagnet heterostructures, pulsed currents can drive morphological transitions between labyrinth-like, stripe-like, and skyrmionic states. Using high-resolution X-ray microscopy, the spin texture evolution with temperature and magnetic field is imaged and it is demonstrated that with transient Joule heating, topological charges can be injected into the system, driving it across the stripe-skyrmion boundary. The observations are explained through atomistic spin dynamic and micromagnetic simulations that reveal a crossover to a global skyrmionic ground state above a threshold magnetic field, which is found to decrease with increasing temperature. It is demonstrated how by tuning the phase stability, one can reliably generate skyrmions by short current pulses and stabilize them at zero field, providing new means to create and manipulate spin textures in engineered chiral ferromagnets.},
 author = {Lemesh, Ivan and Litzius, Kai and B{\"o}ttcher, Marie and Bassirian, Pedram and Kerber, Nico and Heinze, Daniel and Z{\'a}zvorka, Jakub and B{\"u}ttner, Felix and Caretta, Lucas and Mann, Maxwell and Weigand, Markus and Finizio, Simone and Raabe, J{\"o}rg and Im, Mi-Young and Stoll, Hermann and Sch{\"u}tz, Gisela and Dup{\'e}, Bertrand and Kl{\"a}ui, Mathias and Beach, Geoffrey S. D.},
 year = {2018},
 title = {Current-Induced Skyrmion Generation through Morphological Thermal Transitions in Chiral Ferromagnetic Heterostructures},
 pages = {e1805461},
 volume = {30},
 number = {49},
 journal = {Advanced materials (Deerfield Beach, Fla.)},
 doi = {10.1002/adma.201805461},
 file = {6c2e85be-5b57-44e6-a7a5-0952292eeb04:C\:\\Users\\Morris\\AppData\\Local\\Swiss Academic Software\\Citavi 6\\ProjectCache\\k4a9175chg9k578gwv8a52s6g23e9do0zsq8mv1wf6n9yo3cr\\Citavi Attachments\\6c2e85be-5b57-44e6-a7a5-0952292eeb04.pdf:pdf}
}


% This file was created with Citavi 6.8.0.0

@article{Woo.2016,
 abstract = {Magnetic skyrmions are topologically protected spin textures that exhibit fascinating physical behaviours and large potential in highly energy-efficient spintronic device applications. The main obstacles so far are that skyrmions have been observed in only a few exotic materials and at low temperatures, and fast current-driven motion of individual skyrmions has not yet been achieved. Here, we report the observation of stable magnetic skyrmions at room temperature in ultrathin transition metal ferromagnets with magnetic transmission soft X-ray microscopy. We demonstrate the ability to generate stable skyrmion lattices and drive trains of individual skyrmions by short current pulses along a magnetic racetrack at speeds exceeding 100 m s(-1) as required for applications. Our findings provide experimental evidence of recent predictions and open the door to room-temperature skyrmion spintronics in robust thin-film heterostructures.},
 author = {Woo, Seonghoon and Litzius, Kai and Kr{\"u}ger, Benjamin and Im, Mi-Young and Caretta, Lucas and Richter, Kornel and Mann, Maxwell and Krone, Andrea and Reeve, Robert M. and Weigand, Markus and Agrawal, Parnika and Lemesh, Ivan and Mawass, Mohamad-Assaad and Fischer, Peter and Kl{\"a}ui, Mathias and Beach, Geoffrey S. D.},
 year = {2016},
 title = {Observation of room-temperature magnetic skyrmions and their current-driven dynamics in ultrathin metallic ferromagnets},
 pages = {501--506},
 volume = {15},
 number = {5},
 issn = {1476-1122},
 journal = {Nature materials},
 doi = {10.1038/nmat4593},
 file = {a43a49e2-c3c2-4d33-bb1f-700967b9a445:C\:\\Users\\Morris\\AppData\\Local\\Swiss Academic Software\\Citavi 6\\ProjectCache\\k4a9175chg9k578gwv8a52s6g23e9do0zsq8mv1wf6n9yo3cr\\Citavi Attachments\\a43a49e2-c3c2-4d33-bb1f-700967b9a445.pdf:pdf}
}

% This file was created with Citavi 6.8.0.0

@article{Loudon.2019,
 abstract = {The intense research effort investigating magnetic skyrmions and their applications for spintronics has yielded reports of more exotic objects including the biskyrmion, which consists of a bound pair of counter-rotating vortices of magnetization. Biskyrmions have been identified only from transmission electron microscopy images and have not been observed by other techniques, nor seen in simulations carried out under realistic conditions. Here, quantitative Lorentz transmission electron microscopy, X-ray holography, and micromagnetic simulations are combined to search for biskyrmions in MnNiGa, a material in which they have been reported. Only type-I and type-II magnetic bubbles are found and images purported to show biskyrmions can be explained as type-II bubbles viewed at an angle to their axes. It is not the magnetization but the magnetic flux density resulting from this object that forms the counter-rotating vortices.},
 author = {Loudon, James C. and Twitchett-Harrison, Alison C. and Cort{\'e}s-Ortu{\~n}o, David and Birch, Max T. and Turnbull, Luke A. and {\v{S}}tefan{\v{c}}i{\v{c}}, Ale{\v{s}} and Ogrin, Feodor Y. and Burgos-Parra, Erick O. and Bukin, Nicholas and Laurenson, Angus and Popescu, Horia and Beg, Marijan and Hovorka, Ondrej and Fangohr, Hans and Midgley, Paul A. and Balakrishnan, Geetha and Hatton, Peter D.},
 year = {2019},
 title = {Do Images of Biskyrmions Show Type-II Bubbles?},
 pages = {e1806598},
 volume = {31},
 number = {16},
 journal = {Advanced materials (Deerfield Beach, Fla.)},
 doi = {10.1002/adma.201806598},
 file = {180fc2ab-02f2-474d-ad26-c27b538cf37f:C\:\\Users\\Morris\\AppData\\Local\\Swiss Academic Software\\Citavi 6\\ProjectCache\\k4a9175chg9k578gwv8a52s6g23e9do0zsq8mv1wf6n9yo3cr\\Citavi Attachments\\180fc2ab-02f2-474d-ad26-c27b538cf37f.pdf:pdf}
}


% This file was created with Citavi 6.8.0.0

@article{May.2019b,
 author = {May, Andrew F. and Bridges, Craig A. and McGuire, Michael A.},
 year = {2019},
 title = {Physical properties and thermal stability of Fe5$-$xGeTe2 single crystals},
 volume = {3},
 number = {10},
 journal = {Physical Review Materials},
 doi = {10.1103/PhysRevMaterials.3.104401},
 file = {28281468-59fb-4781-90be-929aa0f43209:C\:\\Users\\Morris\\AppData\\Local\\Swiss Academic Software\\Citavi 6\\ProjectCache\\k4a9175chg9k578gwv8a52s6g23e9do0zsq8mv1wf6n9yo3cr\\Citavi Attachments\\28281468-59fb-4781-90be-929aa0f43209.pdf:pdf}
}


% This file was created with Citavi 6.8.0.0

@article{Zhang.2020,
 author = {Zhang, Hongrui and Chen, Rui and Zhai, Kun and Chen, Xiang and Caretta, Lucas and Huang, Xiaoxi and Chopdekar, Rajesh V. and Cao, Jinhua and Sun, Jirong and Yao, Jie and Birgeneau, Robert and Ramesh, Ramamoorthy},
 year = {2020},
 title = {Itinerant ferromagnetism in van der Waals Fe5$-$xGeTe2 crystals above room temperature},
 volume = {102},
 number = {6},
 issn = {2469-9950},
 journal = {Physical Review B},
 doi = {10.1103/PhysRevB.102.064417},
 file = {907fca37-7cb7-4a92-b08d-913d44656c2b:C\:\\Users\\Morris\\AppData\\Local\\Swiss Academic Software\\Citavi 6\\ProjectCache\\k4a9175chg9k578gwv8a52s6g23e9do0zsq8mv1wf6n9yo3cr\\Citavi Attachments\\907fca37-7cb7-4a92-b08d-913d44656c2b.pdf:pdf}
}


% This file was created with Citavi 6.8.0.0

@article{Yokota.2019,
 author = {Yokota, Terufumi},
 year = {2019},
 title = {Numerical Investigation of Magnetic Bubble Types in a Two-Dimensional Ferromagnetic System with Dipole--Dipole Interactions},
 pages = {084702},
 volume = {88},
 number = {8},
 issn = {0031-9015},
 journal = {Journal of the Physical Society of Japan},
 doi = {10.7566/JPSJ.88.084702}
}



% This file was created with Citavi 6.10.0.0

@article{Johansen.2013,
 author = {Johansen, Tom H. and Pan, Alexey V. and Galperin, Yuri M.},
 year = {2013},
 title = {Exact asymptotic behavior of magnetic stripe domain arrays},
 volume = {87},
 number = {6},
 issn = {2469-9950},
 journal = {Physical Review B},
 doi = {10.1103/PhysRevB.87.060402},
 file = {Johansen, Pan et al. 2013 - Exact asymptotic behavior of magnetic:Attachments/Johansen, Pan et al. 2013 - Exact asymptotic behavior of magnetic.pdf:application/pdf}
}


% This file was created with Citavi 6.10.0.0

@article{Ohta.2020,
 author = {Ohta, Tomoharu and Sakai, Kosuke and Taniguchi, Hiroki and Driesen, Benjamin and Okada, Yoshinori and Kobayashi, Kensuke and Niimi, Yasuhiro},
 year = {2020},
 title = {Enhancement of coercive field in atomically-thin quenched Fe 5 GeTe 2},
 pages = {043005},
 volume = {13},
 number = {4},
 issn = {1882-0778},
 journal = {Applied Physics Express},
 doi = {10.35848/1882-0786/ab7f18}
}


% This file was created with Citavi 6.10.0.0

@article{Garanin.1996,
 author = {Garanin},
 year = {1996},
 title = {Self-consistent Gaussian approximation for classical spin systems: Thermodynamics},
 pages = {11593--11605},
 volume = {53},
 number = {17},
 issn = {0163-1829},
 journal = {Physical review. B, Condensed matter},
 doi = {10.1103/physrevb.53.11593},
 file = {Garanin 1996 - Self-consistent Gaussian approximation for classical:Attachments/Garanin 1996 - Self-consistent Gaussian approximation for classical.pdf:application/pdf}
}


% This file was created with Citavi 6.10.0.0

@article{Evans.2014,
 abstract = {Atomistic modelling of magnetic materials provides unprecedented detail about the underlying physical processes that govern their macroscopic properties, and allows the simulation of complex effects such as surface anisotropy, ultrafast laser-induced spin dynamics, exchange bias, and microstructural effects. Here we present the key methods used in atomistic spin models which are then applied to a range of magnetic problems. We detail the parallelization strategies used which enable the routine simulation of extended systems with full atomistic resolution.},
 author = {Evans, R. F. L. and Fan, W. J. and Chureemart, P. and Ostler, T. A. and Ellis, M. O. A. and Chantrell, R. W.},
 year = {2014},
 title = {Atomistic spin model simulations of magnetic nanomaterials},
 pages = {103202},
 volume = {26},
 number = {10},
 journal = {Journal of physics. Condensed matter : an Institute of Physics journal},
 doi = {10.1088/0953-8984/26/10/103202},
 file = {Evans, Fan et al. 2014 - Atomistic spin model simulations:Attachments/Evans, Fan et al. 2014 - Atomistic spin model simulations.pdf:application/pdf}
}


% This file was created with Citavi 6.10.0.0

@article{Stoner.1948,
 year = {1948},
 title = {A mechanism of magnetic hysteresis in heterogeneous alloys},
 pages = {599--642},
 volume = {240},
 number = {826},
 issn = {0080-4614},
 journal = {Philosophical Transactions of the Royal Society of London. Series A, Mathematical and Physical Sciences},
 doi = {10.1098/rsta.1948.0007},
 file = {A mechanism of magnetic hysteresis 1948:Attachments/A mechanism of magnetic hysteresis 1948.pdf:application/pdf}
}









@misc{jukkr,
    author = {{The JuKKR developers}},
    title = {{The J\"ulich KKR Codes}},
    note = {\url{https://jukkr.fz-juelich.de}},
    year = 2021,
}


@article{Ebert2009,
author = {Ebert, H. and Mankovsky, S.},
doi = {10.1103/PhysRevB.79.045209},
issn = {10980121},
journal = {Phys. Rev. B},
number = {4},
pages = {045209},
title = {{Anisotropic exchange coupling in diluted magnetic semiconductors: Ab initio spin-density functional theory}},
volume = {79},
year = {2009}
}


@article{Ebert2011a,
author = {Ebert, H. and K{\"{o}}dderitzsch, D. and Min{\'{a}}r, J.},
doi = {10.1088/0034-4885/74/9/096501},
isbn = {0034-4885},
issn = {00344885},
journal = {Reports Prog. Phys.},
number = {9},
pages = {096501},
title = {{Calculating condensed matter properties using the KKR-Green's function method - Recent developments and applications}},
volume = {74},
year = {2011}
}

@article{Perdew1996,
author = {Perdew, John P. and Burke, Kieron and Ernzerhof, Matthias},
doi = {10.1103/PhysRevLett.77.3865},
file = {:Users/tomsaunderson/Library/Application Support/Mendeley Desktop/Downloaded/Perdew, Burke, Ernzerhof - 1996 - Generalized Gradient Approximation Made Simple.pdf:pdf},
isbn = {9780596529321},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
number = {18},
pages = {3865--3868},
pmid = {10062328},
title = {{Generalized Gradient Approximation Made Simple}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/10062328{\%}5Cnhttp://link.aps.org/doi/10.1103/PhysRevLett.77.3865{\%}5Cnhttp://link.aps.org/abstract/PRL/v77/p3865},
volume = {77},
year = {1996}
}

@article{Liechtenstein1987,
author = {Liechtenstein, A.I. and Katsnelson, M.I. and Antropov, V.P and Gubanov, V.A.},
file = {:Users/tomsaunderson/SeaDrive/Meine Bibliotheken/My Library/2021/Research/Fe5GeTe2/Bulk/FGT{\_}ExchangeConstants/1-s2.0-0304885387907219-main.pdf:pdf},
journal = {J. Magn. Magn. Mater.},
pages = {65--74},
title = {{LOCAL SPIN DENSITY FUNCTIONAL APPROACH TO THE THEORY OF EXCHANGE INTERACTIONS IN FERROMAGNETIC METALS AND ALLOYS A.I. LIECHTENSTEIN, M.I. KATSNELSON +, V.P. ANTROPOV + and V.A. GUBANOV}},
volume = {67},
year = {1987}
}

@article{Schweflinghaus2016,
archivePrefix = {arXiv},
arxivId = {1603.01578},
author = {Schweflinghaus, B. and Zimmermann, B. and Heide, M. and Bihlmayer, G. and Bl{\"{u}}gel, S.},
doi = {10.1103/PhysRevB.94.024403},
eprint = {1603.01578},
file = {:Users/tomsaunderson/Library/Application Support/Mendeley Desktop/Downloaded/Schweflinghaus et al. - 2016 - Role of Dzyaloshinskii-Moriya interaction for magnetism in transition-metal chains at Pt step edges.pdf:pdf},
issn = {24699969},
journal = {Phys. Rev. B},
number = {2},
pages = {024403},
title = {{Role of Dzyaloshinskii-Moriya interaction for magnetism in transition-metal chains at Pt step edges}},
volume = {94},
year = {2016}
}

@article{Stefanou1991,
author = {Stefanou, N. and Zeller, R.},
doi = {10.1088/0953-8984/3/39/006},
file = {:Users/tomsaunderson/SeaDrive/Meine Bibliotheken/My Library/2021/Research/Fe5GeTe2/Bulk/N{\_}Stefanou{\_}1991{\_}J.{\_}Phys. {\_}Condens.{\_}Matter{\_}3{\_}7599.pdf:pdf},
issn = {09538984},
journal = {J. Phys. Condens. Matter},
number = {39},
pages = {7599--7606},
title = {{Calculation of shape-truncation functions for Voronoi polyhedra}},
volume = {3},
year = {1991}
}

@article{Stefanou1990,
author = {Stefanou, N. and Akai, H. and Zeller, R.},
doi = {10.1016/0010-4655(90)90009-P},
file = {:Users/tomsaunderson/SeaDrive/Meine Bibliotheken/My Library/2021/Research/Fe5GeTe2/Bulk/1-s2.0-001046559090009P-main.pdf:pdf},
issn = {00104655},
journal = {Comput. Phys. Commun.},
number = {2},
pages = {231--238},
title = {{An efficient numerical method to calculate shape truncation functions for Wigner-Seitz atomic polyhedra}},
volume = {60},
year = {1990}
}


% This file was created with Citavi 6.10.0.0

@article{Alahmed.2021,
 author = {Alahmed, Laith and Nepal, Bhuwan and Macy, Juan and Zheng, Wenkai and Casas, Brian and Sapkota, Arjun and Jones, Nicholas and Mazza, Alessandro R. and Brahlek, Matthew and Jin, Wencan and Mahjouri-Samani, Masoud and Zhang, Steven S.-L. and Mewes, Claudia and Balicas, Luis and Mewes, Tim and Li, Peng},
 year = {2021},
 title = {Magnetism and spin dynamics in room-temperature van der Waals magnet Fe 5 GeTe 2},
 pages = {045030},
 volume = {8},
 number = {4},
 journal = {2D Materials},
 doi = {10.1088/2053-1583/ac2028},
 file = {Alahmed, Nepal et al. 2021 - Magnetism and spin dynamics:Attachments/Alahmed, Nepal et al. 2021 - Magnetism and spin dynamics.pdf:application/pdf}
}

@article{doi:10.1021/acsnano.8b09660,
author = {May, Andrew F. and Ovchinnikov, Dmitry and Zheng, Qiang and Hermann, Raphael and Calder, Stuart and Huang, Bevin and Fei, Zaiyao and Liu, Yaohua and Xu, Xiaodong and McGuire, Michael A.},
title = {Ferromagnetism Near Room Temperature in the Cleavable van der Waals Crystal Fe5GeTe2},
journal = {ACS Nano},
volume = {13},
number = {4},
pages = {4436-4442},
year = {2019},
doi = {10.1021/acsnano.8b09660},
    note ={PMID: 30865426},
URL = { 
        https://doi.org/10.1021/acsnano.8b09660
},
eprint = { 
        https://doi.org/10.1021/acsnano.8b09660
    }
}

@article{Muller2019,
abstract = {The Spirit framework is designed for atomic-scale spin simulations of magnetic systems with arbitrary geometry and magnetic structure, providing a graphical user interface with powerful visualizations and an easy-to-use scripting interface. An extended Heisenberg-type spin-lattice Hamiltonian including competing exchange interactions between neighbors at arbitrary distances, higher-order exchange, Dzyaloshinskii-Moriya and dipole-dipole interactions is used to describe the energetics of a system of classical spins localized at atom positions. A variety of common simulation methods are implemented including Monte Carlo and various time evolution algorithms based on the Landau-Lifshitz-Gilbert (LLG) equation of motion. These methods can be used to determine static ground-state and metastable spin configurations, sample equilibrium and finite-temperature thermodynamical properties of magnetic materials and nanostructures, or calculate dynamical trajectories including spin torques induced by stochastic temperature or electric current. Methods for finding the mechanism and rate of thermally assisted transitions include the geodesic nudged elastic band method, which can be applied when both initial and final states are specified, and the minimum mode-following method when only the initial state is given. The lifetimes of magnetic states and rates of transitions can be evaluated within the harmonic approximation of transition-state theory. The framework offers performant central processing unit (CPU) and graphics processing unit (GPU) parallelizations. All methods are verified and applications to several systems, such as vortices, domain walls, skyrmions, and bobbers are described.},
author = {M{\"{u}}ller, Gideon P and Hoffmann, Markus and Di{\ss}elkamp, Constantin and Sch{\"{u}}rhoff, Daniel and Mavros, Stefanos and Sallermann, Moritz and Kiselev, Nikolai S and J{\'{o}}nsson, Hannes and Bl{\"{u}}gel, Stefan},
doi = {10.1103/PhysRevB.99.224414},
file = {:C\:/Users/Tom/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/M{\"{u}}ller et al. - 2019 - Spirit Multifunctional framework for atomistic spin simulations(2).pdf:pdf},
journal = {Phys. Rev. B},
keywords = {doi:10.1103/PhysRevB.99.224414 url:https://doi.org},
pages = {224414},
title = {{Spirit: Multifunctional framework for atomistic spin simulations}},
url = {https://juspin.de;g.mueller@fz-juelich.de},
volume = {99},
year = {2019}
}

@article{Skubic2008,
abstract = {We present a method for performing atomistic spin dynamic simulations. A comprehensive summary of all pertinent details for performing the simulations such as equations of motions, models for including temperature, methods of extracting data and numerical schemes for performing the simulations is given. The method can be applied in a first-principles mode, where all interatomic exchange is calculated self-consistently, or it can be applied with frozen parameters estimated from experiments or calculated for a fixed spin-configuration. Areas of potential application to different magnetic questions are also discussed. The method is finally applied to one situation where the macrospin model breaks down; magnetic switching in ultra strong magnetic fields. {\textcopyright} IOP Publishing Ltd.},
archivePrefix = {arXiv},
arxivId = {0806.1582},
author = {Skubic, B. and Hellsvik, J. and Nordstr{\"{o}}m, L. and Eriksson, O.},
doi = {10.1088/0953-8984/20/31/315203},
eprint = {0806.1582},
file = {:C\:/Users/Tom/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Skubic et al. - 2008 - A method for atomistic spin dynamics simulations implementation and examples.pdf:pdf},
issn = {0953-8984},
journal = {J. Phys. Condens. Matter},
month = {jul},
number = {31},
pages = {315203},
publisher = {IOP Publishing},
title = {{A method for atomistic spin dynamics simulations: implementation and examples}},
url = {https://iopscience.iop.org/article/10.1088/0953-8984/20/31/315203 https://iopscience.iop.org/article/10.1088/0953-8984/20/31/315203/meta},
volume = {20},
year = {2008}
}

@article{Heide2008a,
abstract = {Combining relativistic first-principles calculations with a micromagnetic model, we establish the Dzyaloshinskii-Moriya interaction as an important mechanism in thin-film magnetism, determining the orientation of magnetic domains relative to the lattice, the type of domain wall, and the rotational direction of the magnetization in the wall. Applying the analysis to two monolayers Fe on W(110), we provide an explanation for puzzling experimental data obtained by spin-polarized scanning tunneling microscopy. {\textcopyright} 2008 The American Physical Society.},
author = {Heide, M. and Bihlmayer, G. and Bl{\"{u}}gel, S.},
doi = {10.1103/PHYSREVB.78.140403/FIGURES/5/MEDIUM},
file = {:E\:/Users/Tom/seadrive_root/Thomas G/My Libraries/My Library/2021/Research/Fe5GeTe2/PhysRevB.78.140403.pdf:pdf},
issn = {10980121},
journal = {Phys. Rev. B},
month = {oct},
number = {14},
pages = {140403},
publisher = {American Physical Society},
title = {{Dzyaloshinskii-Moriya interaction accounting for the orientation of magnetic domains in ultrathin films: Fe/W(110)}},
url = {https://journals.aps.org/prb/abstract/10.1103/PhysRevB.78.140403},
volume = {78},
year = {2008}
}

% This file was created with Citavi 6.10.0.0

@article{Sherrington.1975,
 author = {Sherrington, David and Kirkpatrick, Scott},
 year = {1975},
 title = {Solvable Model of a Spin-Glass},
 pages = {1792--1796},
 volume = {35},
 number = {26},
 issn = {0031-9007},
 journal = {Physical Review Letters},
 doi = {10.1103/PhysRevLett.35.1792}
}

% This file was created with Citavi 6.10.0.0

@article{VOLKL.1995,
 author = {V{\"O}LKL, E. and ALLARD, L. F. and FROST, B.},
 year = {1995},
 title = {A software package for the processing and reconstruction of electron holograms},
 pages = {39--50},
 volume = {180},
 number = {1},
 issn = {00222720},
 journal = {Journal of Microscopy},
 doi = {10.1111/j.1365-2818.1995.tb03655.x}
}






